Optimizing the MapReduce Framework on Intel Xeon Phi Coprocessor

With the ease-of-programming, flexibility and yet efficiency, MapReduce has become one of the most popular frameworks for building big-data applications. MapReduce was originally designed for distributed-computing, and has been extended to various architectures, e,g, multi-core CPUs, GPUs and FPGAs. In this work, we focus on optimizing the MapReduce framework on Xeon Phi, which is the latest product released by Intel based on the Many Integrated Core Architecture. To the best of our knowledge, this is the first work to optimize the MapReduce framework on the Xeon Phi. In our work, we utilize advanced features of the Xeon Phi to achieve high performance. In order to take advantage of the SIMD vector processing units, we propose a vectorization friendly technique for the map phase to assist the auto-vectorization as well as develop SIMD hash computation algorithms. Furthermore, we utilize MIMD hyper-threading to pipeline the map and reduce to improve the resource utilization. We also eliminate multiple local arrays but use low cost atomic operations on the global array for some applications, which can improve the thread scalability and data locality due to the coherent L2 caches. Finally, for a given application, our framework can either automatically detect suitable techniques to apply or provide guideline for users at compilation time. We conduct comprehensive experiments to benchmark the Xeon Phi and compare our optimized MapReduce framework with a state-of-the-art multi-core based MapReduce framework (Phoenix++). By evaluating six real-world applications, the experimental results show that our optimized framework is 1.2X to 38X faster than Phoenix++ for various applications on the Xeon Phi.

==> impl-lei.tex <==

\section{MRPhi: An Optimized MapReduce Framework on Xeon Phi} \label{sec:mrphi}

In this section, we present our proposed MapReduce framework \textit{MRPhi}, which is specially optimized for the Intel Xeon Phi coprocessor.

\subsection{Overview}

MRPhi adopts state-of-the-art techniques from the shared memory MapReduce framework as well as specific optimizations for the Xeon Phi coprocessor. Overall, we adopt the similar design as Phoenix++ \cite{phoenix++} to implement the basic MapReduce workflow as shown in Figure \ref{fig:basic_workflow}. There are two major techniques from Phoenix++ adopted in our framework, which are efficient combiners and different container structures. We briefly introduce the two techniques and refer readers to the original Phoenix++ paper \cite{phoenix++} for more details.
\begin{itemize}
\item{\textit{Efficient combiners}. Each map worker maintains a local container. When an intermediate key-value pair is generated by a map function, the reduce operator is immediately applied to that pair based on the local container. This process is performed using a \textit{combiner}. Therefore, a map operation essentially consists of two parts, which are the computation defined in the map function and combiner execution. After that, the partition is applied to each local container and multiple local containers are merged to a global container in the reduce phase. Our MRPhi adopts this similar design. However, one of our technique is to eliminate the local containers (Section \ref{sec:global}) in some cases.}
\item{\textit{Hash table and array containers}. MRPhi supports two data structures for containers, which are hash table and array. The array container is efficient when the keys are integers and in a fixed range.}
\end{itemize}

\begin{figure}[ht]
\centering
\includegraphics[scale=0.35]{figure/opt_tech}
\vspace*{-.0cm}
\caption{Proposed techniques in MRPhi.}
\label{fig:opt_tech} \vspace*{-.3cm}
\end{figure}


In addition to the similar design as Phoenix++, we propose four effective optimization techniques for the Xeon Phi. Note that these techniques are not applicable for all cases. Figure \ref{fig:opt_tech} summarizes the techniques and their suitability. We introduce them briefly here and will present the detail in the following sections.

\textbf{Pipelining of map and reduce phases.} In general, the map phase is computation-intensive, and the reduce phase is memory-intensive. In order to better utilize the hardware resource with hyperthreading, we pipeline the map and reduce phases. This technique is effective for the hash table container.

\textbf{SIMD hash computation.} For the hash table container, we can utilize SIMD instructions to implement the hash computation efficiently.

\textbf{Vectorization friendly map.} MRPhi implements the map phase in a vectorization friendly way, which clears the dependency among map operations. This way, the compiler can effectively vertorize multiple map operations to take advantage of VPUs.

\textbf{Global array with atomic operations.} For the array container, if the array is very large, it introduces a number of performance issues because of local arrays adopted. We address these issues by eliminating local arrays but employing low overhead atomic operations.


\subsection{Pipelined Map and Reduce Phases} \label{sec:pipeline}


\reminder{consider to shorten this section, as not so effective}

As introduced in Section \ref{sec:issue}, one of the performance issues of Phoenix++ is the high memory latency when building hash tables. There are rich studies to hide the latency for hash table building through prefetching \cite{chen04, zhou05}. For MRPhi, we adopt prefetching instructions to achieve the similar purpose. Furthermore, we adopt another technique specifically for the MapReduce framework, which is to pipeline the map and reduce phases. The motivation is that the map function defined by users usually contains computation-intensive workloads. Instead, the reduce phase is memory-intensive in most cases since the reduce operator is usually simple, such as the addition. This way, the computation-intensive map and memory-intensive reduce are concurrently executed to improve the overall hardware resource utilization. This technique is more effective for the hash table container. Since for the array container, the time of reduce phase is usually insignificant compared with the map phase.

\begin{figure}[ht]
\centering
\includegraphics[scale=0.35]{figure/pipeline}
\vspace*{-.0cm}
\caption{The producer-consumer model for the pipelined map and reduce phases.}
\label{fig:pipeline} \vspace*{-.3cm}
\end{figure}

We design an efficient producer-consumer model to pipeline the map and reduce phases. There are three major data structures, which are local hash tables, a global hash table, and partition queues. Specifically, each map worker still has a local hash table. However, the local table works on a pre-allocated fix-sized small buffer. This is to improve the data locality of local hash table building. There are First-In-First-Out queues for different partitions. The \textit{push} and \textit{pop} operations on the queues are performed by the map and reduce workers, respectively. Suppose there are $N_r$ reduce workers, then there are $N_r$ queues.

Figure \ref{fig:pipeline} illustrates an example of three producers and three consumers. There are concurrent map workers (\textit{MWorker}) and reduce workers (\textit{RWorker}) on each core. It works in this way. Each map worker processes the data and builds its own local hash table. When the local hash table is full (the underlying fix-sized buffer is full), it partitions the table and send partition $i$ to queue $i$. After that, the local table becomes empty, and the map worker continues the processing. On the other hand, each reduce work takes charges of one queue. As long as the queue is non-empty, it fetches the partitions and builds the global hash table. Since data are partitioned, there is no conflicts among reduce workers.

In our model, we restrict the memory accesses of each local table building on a fix-sized small buffer. We make the overall size of these buffers on the same core smaller than the L2 cache. This can reduce the memory latency for the map phase and make it be more likely computation-bound. On the other hand, the reduce phase is memory latency bound. We pipeline the map and reduce phases to better utilize the hardware resource. Of course, this model introduces storage overhead compared with the non-pipelined model. Nevertheless, this technique is worthwhile when the workloads of the map computation and hash table building are similar. By evaluating real-world applications and data sets, it is useful to improve the performance.

\subsection{SIMD Hash Computation} \label{sec:hash}
The SIMD feature of Intel Xeon Phi offers tremendous computing power by executing a vector of computation simultaneously.
The supported 512-bit SIMD instructions can either operate on single/double-precision floating point numbers
or integers. For example, the SIMD hardware unit can process a vector of 16 integer computation simultaneously. Hash computation is a key component in the MapReduce framework as it has to be invoked for every key-value pair. In this section, we evaluate the efficiency of SIMD operations on hash computation and investigate the optimization issues.

There have been many hash functions used for MapReduce framework. Among them, we choose the one that can be implemented using SIMD instructions (e.g., the hash function does not involve complex control flow). The hash function accepts a string as parameter and returns an integer as the hash value. We choose 32-bit hash value as Intel Xeon Phi's SIMD unit has relatively limited support for 64-bit integer computations. The pseudo hash function is shown in Listing~\ref{list:1}. The hash algorithm is simple. It just iterates through the string and performs computation for each character. The final hash value depends on every character of the string. The computation pattern is simple and can be easily implemented using SIMD instructions.

\begin{lstlisting}[language=C,frame=shadowbox,caption=Original PTX code,captionpos=b,numbers=left,xrightmargin=9pt,xleftmargin=9pt,breaklines=true,tabsize=2]
uint32_t BKDR(char *str) {
uint32_t seed = 131; // 31 131 1313 13131 131313 etc..
uint32_t hash = 0;
while (*str) {
        hash = hash * seed + (*str++);
}
return (hash & 0x7FFFFFFF);
}
\end{lstlisting}\label{list:1}

Table~\ref{table:simd} gives the widely used SIMD instructions for 32-bit integers. Note that, for all the SIMD instructions, 
Xeon Phi provides a corresponding mask version. The mask version can selectively execute only a portion of vector using mask.  

\begin{table*}[ht] \small
\begin{center}  \caption{\small SIMD Instruction}\vspace*{.1cm}
\label{table:simd}
    \begin{tabular}{|l|c|}
        \hline\hline
        \textbf{Compiler Intrinsic} & \textbf{Description} \\
        \hline
        \_mm512\_load\_epi32 & Loads 16 32-bit integer values from memory address into int32 vector. \\
        \hline
        \_mm512\_i32gather\_epi32 & Gather a set of 16 memory locations with scale into an int32 vector. \\
        \hline
        \_mm512\_add\_epi32 & Performs an element-by-element addition between two int32 vectors. \\
        \hline
        \_mm512\_mullo\_epi32 & Performs an element-by-element multiplication between two int32 vectors. \\
        \hline
        \_mm512\_and\_epi32 & Performs a bitwise AND operation between two int32 vectors. \\
        \hline
    \end{tabular}
\end{center}
\end{table*}

We propose two different SIMD implementations with different implementation and performance overhead. 
The first one is easy to implement, but may lead to low SIMD hardware utilization. The second one improves 
the SIMD hardware utilization but at expense of complex control flow overhead. 
In the following, we name these two implementations as SIMDHash1 and SIMDHash2.

\subsubsection{SIMDHash1}
For the first implementation, it processes a vector of 16 int32s in parallel. In other words, in each round, the hash 
function processes 16 strings in parallel and generates 16 int32s. The pseudo code of the implementation is shown in Listing~\ref{list:2}.
At line 1, we use the gather instruction to load 16 characters into the int32 vector. Note that each character is a 8-bit integer, so we need a conversion from int8 to int32 to load 16 characters into a vector of int32s. At line 3, we do a SIMD comparison to test whether each character is equal to zero, i.e., the terminating character. If yes, it means the corresponding string finishes its computation. If all the 16 strings finish the computation, then we proceed to the next group. At line 7, we utilize the SIMD fused-multiply-add instruction to combine the multiplication and addition operations in the original hash function into one operation. At line 8, we increment the index of characters so we can proceed to the next character in each of the 16 strings.

\begin{lstlisting}[language=C,frame=shadowbox,caption=Original PTX code,captionpos=b,numbers=left,xrightmargin=9pt,xleftmargin=9pt,breaklines=true,tabsize=2]
chars.reg = _mm512_i32extgather_epi32(_mm512_add_epi32(offs.reg, idxs.reg), ....);
__mmask16 mask = _mm512_cmpneq_epi32_mask(chars.reg, zeros.reg);
if (_mm512_kortestz(mask, mask))
	break;
hashes.reg = _mm512_mask_fmadd_epi32(hashes.reg, mask, seeds.reg, chars.reg);
idxs.reg = _mm512_mask_add_epi32(idxs.reg, mask, idxs.reg, ones.reg);

\end{lstlisting}\label{list:2}

Let us use an example to explain how SIMDHash1 works. For simplicity, let us assume the SIMD unit is 2-way instead of 16-way, which means it can process 2 integers in parallel. Given the input sentence "This is Xeon Phi", Figure~\ref{fig:simd1} shows how we compute hash values for the 4 words in this sentence.
The sentence "This is Xeon Phi" is divided into two groups. The first group is composed of the words 'This' and 'is', the second composed of 'Xeon' and 'Phi'.
SIMD units attempts to process two characters in each round. If different words have different lengths (e.g., this and is), then we use mask to indicate which word has finished its computation. Obviously, the SIMD hardware unit may be wasted if different words have different lengths.

\begin{figure}[ht]
\centering
\includegraphics[scale=0.56]{figure/simd1.pdf}
\vspace*{-.0cm}
\caption{SIMDHH-padding Implementation.}
\label{fig:simd1} \vspace*{-.3cm}
\end{figure}

\subsubsection{SIMDHash2}
To improve the SIMD hardware utilization, we devise the SIMDHash2. In SIMDHash2, we do not divide the array of words in to groups. Instead, we just continuously feed the SIMD unit with strings. The processed character for each iteration of previous example is shown in Figure~\ref{fig:simd2}.

\begin{figure}[ht]
\centering
\includegraphics[scale=0.56]{figure/simd2.pdf}
\vspace*{-.0cm}
\caption{SIMDHash2 Implementation.}
\label{fig:simd2} \vspace*{-.3cm}
\end{figure}

In this implementation, we still process two words in parallel each time. First, we start to process words "This" and "is". In the 3rd iteration, the word "is" in the second unit is finished. This time, however, we don't wait for the word "this" in the first unit to finish. We just pack the next word "Xeon" into the second unit and continue the process. In the 5th iteration, the word "This" is also finished, and we can pack "Phi" into the first unit. In this implementation, we can finish the computation of 4 words in 9 iterations, compared to 10 iterations in SIMDHash1. When the words are more variant in terms of lengths, the difference in number of iterations required by SIMDHash1 and SIMDHash2 are more significant.

However, we reduce the number of iterations as the expense of control flow overhead. Even a simple control flow may lead to complex implementation in SIMD fashion. In SIMDHash1, in each iteration, we only need to check if the 16 characters in the vector are equal to zero. If that's true for all 16 characters, then we know the current group is finished and we can proceed to the next group. In SIMDHash2, however, we not only need to check if each character is zero, but we also have to decide what to do if it is zero. Consider the 3rd iteration in Figure~\ref{fig:simd2}. First, we check the character in the first element. It's not zero, so nothing need be done. Then we check the second element. It's zero, so we should pack in the next unprocessed word, which is "Xeon". We have to check the first element before the second one. Assume we're in the ith iteration, and the next unprocessed string is the kth of the array of strings. If both the first and second element in the SIMD vector is done, we should pack the kth string into the first element, and (k+1)th for the second. But if only the second element is done, we then pack the kth string into the second element. So the string to pack into the second element depends on the status of the second element. Thus this checking process is serial. 

To minimize the overhead, we use a prefix-sum instruction. The prefix-sum of a sequence of numbers x0, x1, x2, ... is a second sequence of numbers y0, y1, y2, ..., the sums of prefixes (running totals) of the input sequence:

\begin{lstlisting}[language=C,frame=shadowbox,caption=Original PTX code,captionpos=b,numbers=left,xrightmargin=9pt,xleftmargin=9pt,breaklines=true,tabsize=2]
y0 = x0
y1 = x0 + x1
y2 = x0 + x1 + x2
y3 = x0 + x1 + x2 + x3
...
\end{lstlisting}\label{list:3}

We compute the prefix-sum using lookup-table. We can store the prefix-sum of each possible vector in a table in advance. And then we can directly get the prefix-sum for an arbitrary vector from the table. As we need to compute prefix-sum of a vector of 16 elements (result of a SIMD comparison), each element being 0 or 1, there would be $2^16$ different cases of input, thus $2^16$ entries is needed in the lookup-table. If each entry is array of 16 8-bit integers, we need 1MB of memory to store the table, which exceeds the cache size. To reduce the size of the table, we can divide the vector of 16 elements into 2 sub-vectors, each composed of 8 elements. Then we can compute the prefix-sum of the 16-sized vector in two steps, each step computing the prefix-sum of a 8-sized vector, and combine the result in the final step. In this way, only a lookup-table of $2^8$ entries is needed, which is about 2KB in memory.

To compute the prefix-sum, we need to divide a vector of 16 elements into 2 sub-vectors and combine the result later. This process requires more than 4 SIMD instructions, during which 2 memory accesses is issued. From our experiment, the prefix-sum method is even slower than directly using a loop of 16 iterations(checking 16 elements one by one). We compare the performance of both SIMDHash1 and SIMDHash2 with the original hash function, operating on a large array of words. SIMDHash1 achieves about 3.5x speedup over the naive hash, and SIMDHash2 gets a speedup of about 2.3x. Although SIMDHash2 is more efficient than SIMDHash1 in theory, but it also has more complex control flow, which is not easy for SIMD implementation. Hence, in practice SIMDHash1 has better performance.

\subsection{Vectorization Friendly Map}

Utilizing VPUs (either by SIMD instructions or vectorization) is critical to high-performance on the Xeon Phi coprocessor. However, for the MapReduce framework itself, in addition to the hash computation, there is little chance to employ SIMD instructions. On the other hand, the user-defined map function has the possibility for vectorization. There are two cases for a map function, which are containing loops or no loop. For the first case, we completely leave the compiler to identify the vectorization within the map function. We propose a technique to help the vectorization for the second case. This technique is applicable to either hash table or array container.


Recall that each thread (or map worker) processes a number of map operations. The computation in those map operations is independent with each other. This provides the opportunity to parallelze multiple map operations by vectorization. The following code demonstrates the basic idea. The \textit{\#pragma ivdep} tells the compiler to vectorize this for-loop if there is no dependency. \\
\line(1,0){250}
\lstset{basicstyle=\footnotesize\ttfamily, language=c++}
\begin{lstlisting}
//N: the number of map operations in the worker
//elems: the input array
#pragma ivdep
for(i = 0; i < N; i++) {
    //the inlined map function
    map(data_t elems[i]) {
        ... //some computation
        emit_intermediate(key, value);
        ...
    }
}
\end{lstlisting}
\vspace{-0.4cm}
\line(1,0){250}





However, in Phoenix++, the \textit{emit\_intermediate} statement introduces dependency, which will make the vectorization failed. For each \textit{emit\_intermediate}, the combiner is performed based on a local container. Concurrent updates on a local container will cause conflicts. This dependency exists for either array or hash table containers. We take the array container as an example. Figure \ref{fig:vectorization_friendly_a} illustrates an example that map operations are failed to be vectorized due to the dependency of \textit{emit\_intermediate}.


\begin{figure}
\subfigure[The original design of map operations with dependency
]{\includegraphics[scale=0.3]{figure/vectorization_friendly_a} \label{fig:vectorization_friendly_a}}
\vfill \subfigure[Vectoriation friendly map]{\includegraphics[scale=0.3]{figure/vectorization_friendly_b} \label{fig:vectorization_friendly_b}}
\caption{Comparison of different designs for the map phase.}
\label{fig:vectorization_friendly}
\end{figure}

We propose a vectorization friendly technique to address this issue. Instead of performing the combiner for each intermediate pair generated by \textit{emit\_intermediate} immediately, we buffer a number of pairs. Writing to the buffer is independent for each map operation. When the buffer is full, we call the combiner for those pairs sequentially. Figure \ref{fig:vectorization_friendly_b} demonstrates this vectorization friendly map. Our vectorization friendly map clears the dependency among map operations to assist the vectorization by the compiler.



\subsection{Global Array with Atomic Operations} \label{sec:global}



Recall that Phoenix++ adopts a local container for each worker in the map phase. Then the local containers are merged in the reduce phase to the final result. This design is efficient when the container size is small. However, it will introduce a number of performance issues when the container becomes large, especially on the Xeon Phi with limited memory size.

An alternative is to eliminate local containers, but directly update on the global container with low-cost atomic operations (if applicable). This technique is effective for the array container. Since the atomic data types only support basic arithmetics. The hash table usually requires more complex data types and operations, such as text strings and memory allocation. Thanks to the low overhead of atomic data types on the Xeon Phi, using the global array directly is more efficient when the array becomes large. There are four advantages of employing the global array with atomic operations instead of local arrays when the array size is large.

\textbf{Thread scalability.} Due to the relatively small memory size on the Xeon Phi (8 GB), the thread scalability can be limited when using local arrays. Suppose the local array size is $L$ bytes, the available memory is $M$ bytes, then the maximum number of concurrent threads for the map phase is $\lfloor{\frac{M}{L}\rfloor}$. As an extreme example of using Bloom filter in bioinformatics \cite{bloomfilter} (evaluated in Section \ref{sec:experiment}), if the whole human genome is used, the local array size is around 3.7 GB. In such a case, only two threads can be used on the Xeon Phi employing local arrays. Instead, using the global array does not have this issue as long as the global array can fit into the memory.

\textbf{Cache efficiency.} When the array is small to fit into the L2 cache, using local arrays has good cache efficiency. However, when the array becomes large, random memory accesses on local arrays cause poor data locality. Using the global array directly is able to improve the cache efficiency by the ring interconnection for L2 caches on the Xeon Phi. Specifically, when using local arrays, every L2 local cache miss should cause a memory access. On the contrary, when using the global array directly, the global array is shared across multiple cores. When a L2 cache miss occurs on the local core, the data may be copied from another core's L2 cache to avoid the expensive memory access. This takes advantage of the ring-based interconnection architecture on the Xeon Phi.

\textbf{The reduce phase time.} Since the intermediate pairs generated by the map phase are directly applied to the global array, the reduce phase is eliminated. This also helps the performance when the array is large.

\textbf{Memory initialization overhead.} We find that the memory initialization is expensive on the Xeon Phi, which happens when the memory space is first touched within a program. Therefore, with the reduced memory footprint by eliminating local arrays, our technique can significantly reduce the overhead of memory initialization.



